Automating System Test Case Classification and Prioritization for Use Case-Driven Testing in Product Lines

Product Line Engineering (PLE) is a crucial practice in many software development environments where software systems are complex and developed for multiple customers with varying needs. At the same time, many development processes are use case-driven and this strongly influences their requirements engineering and system testing practices. In this paper, we propose, apply, and assess an automated system test case classification and prioritization approach specifically targeting system testing in the context of use case-driven development of product families. Our approach provides: (i) automated support to classify, for a new product in a product family, relevant and valid system test cases associated with previous products, and (ii) automated prioritization of system test cases using multiple risk factors such as fault-proneness of requirements and requirements volatility in a product family. Our evaluation was performed in the context of an industrial product family in the automotive domain. Results provide empirical evidence that we propose a practical and beneficial way to classify and prioritize system test cases for industrial product lines.

==> algos/algodiff.tex <==
\begin{tiny}
\begin{algo}

\DontPrintSemicolon 
 \SetKwInOut{Input}{Inputs}\SetKwInOut{Output}{Output}
 \SetAlgoLined
  \SetInd{0.6em}{0.6em}
 \setcounter{AlgoLine}{0}
\Input{Decision model, $M1$, Decision model, $M2$\\}
 \Output{Set of sets of decision-level changes}
 \BlankLine
 
%\textit{\color{darkgreen} /* UC Diagrams*/} \;
Let $\mathit{d}$ be a pair $(vp, uc)$ such that $vp$ is a variation point and $uc$ is a use case including $vp$;\;
Let $\mathit{s}$ be a pair $(uc, fl)$ such that $uc$ is a use case and $fl$ is an optional alternative flow in $uc$;\;
Let $\mathit{p}$ be a triple $(uc, fl, st)$ such that $uc$ is a use case, $fl$ is a flow in $uc$, and $st$ is a step in $fl$;\;
Let $\mathit{D1}$ and $\mathit{D2}$ be the sets of pairs $d$ in $\mathit{M1}$ and $\mathit{M2}$;\;
%Let $\mathit{DD2}$ be the set of tuples $d$ in $\mathit{DM2}$;\;
Let $\mathit{S1}$ and $\mathit{S2}$ be the sets of pairs $s$ in $\mathit{M1}$ and $\mathit{M2}$;\;
%Let $\mathit{SP2}$ be the set of tuples $s$ in $\mathit{DM2}$;\;
Let $\mathit{P1}$ and $\mathit{P2}$ be the sets of triples $p$ in $\mathit{M1}$ and $\mathit{M2}$;\;
%Let $\mathit{SP2}$ be the set of triples $p$ in $\mathit{DM2}$;\;
Let $\mathit{E1}$ and $\mathit{E2}$ be the sets of entities in $\mathit{M1}$ and $\mathit{M2}$;\;
%Let $\mathit{DE2}$ be the set of domain entities in $\mathit{DM2}$;\;
%Let $\mathit{SP3}$, $\mathit{DE2}$ and $\mathit{DE3}$ be the empty sets;\;
%Let $\mathit{DE3}$ be the empty set;\; %for the non-matching domain entities in $\mathit{DM1}$;\;
%Let $\mathit{DEL}$ be the empty set for the deleted decisions;\;
%Let $\mathit{ADD}$ be the empty set for the added decisions;\;
%Let $\mathit{UPDATE}$ be the empty set for updated decisions;\;
$\mathit{D3}\leftarrow$ \textbf{matchDiagramDecisions}($\mathit{D1}$, $\mathit{D2}$);\;
$\mathit{S3} \leftarrow$ \textbf{matchFlowDecisions}($\mathit{S1}$, $\mathit{S2}$);\;
$\mathit{P3} \leftarrow$ \textbf{matchStepDecisions}($\mathit{P1}$, $\mathit{P2}$);\;
$\mathit{E3} \leftarrow$ \textbf{matchDomainModelDecisions}($\mathit{E1}$, $\mathit{E2}$);\;

%\textit{\color{darkgreen} /* Use Case Diagram*/} \;
%$\mathit{DELETE} \leftarrow \mathit{D1}\,\backslash\, \mathit{D3} $;\,\,\,\,\, $\mathit{ADD} \leftarrow \mathit{D2}\,\backslash\, \mathit{D3} $;\;
$\mathit{DELETE} \leftarrow (\mathit{D1}\,\backslash\, \mathit{D3})\, \cup\, (\mathit{S1}\,\backslash\, \mathit{S3}) \, \cup\, (\mathit{P1}\,\backslash\, \mathit{P3})$;\;
$\mathit{ADD} \leftarrow (\mathit{D2}\,\backslash\, \mathit{D3})\, \cup\,(\mathit{S2}\,\backslash\, \mathit{S3}) \,  \cup\,(\mathit{P2}\,\backslash\, \mathit{P3})$;\;
\ForEach{$(k \in (\mathit{D3} \, \cap \mathit{D1}))$}
{
$\mathit{z} \leftarrow$ \textbf{getMatchingDecision}($\mathit{k}$, $\mathit{D3}$);\;
$\mathit{SUC1} \leftarrow$ \textbf{getSelectedUseCases}($\mathit{k}$, $\mathit{M1}$);\;
$\mathit{SUC2} \leftarrow$ \textbf{getSelectedUseCases}($\mathit{z}$, $\mathit{M2}$);\;

\If{($SUC1 \neq SUC2$)}
{$\mathit{UPDATE} \leftarrow \mathit{UPDATE} \,\cup\,\{k\}$;\;}

}

%\textit{\color{darkgreen} /* Use Case Specifications*/} \;

\ForEach{$(t \in (\mathit{S3} \, \cap \mathit{S1}))$}
{
$\mathit{y} \leftarrow$ \textbf{getMatchingDecision}($\mathit{t}$, $\mathit{S3}$);\;

\If{($t.fl.isSelected \neq y.fl.isSelected$)}
{$\mathit{UPDATE} \leftarrow \mathit{UPDATE} \,\cup\,\{t\}$;\;}
}


{


\ForEach{$(u \in (\mathit{P3} \, \cap \mathit{P1}))$}
{
$\mathit{m} \leftarrow$ \textbf{getMatchingDecision}($\mathit{u}$, $\mathit{P3}$);\;

\eIf{($u.st \, \textbf{is} \, OptionalStep$) \textbf{and} ($u.st.isSelected \neq m.st.isSelected$)}
{$\mathit{UPDATE} \leftarrow \mathit{UPDATE} \,\cup\,\{u\}$;\;}
{

\If{($u.st.orderNumber \neq m.st.orderNumber$)}
{$\mathit{UPDATE} \leftarrow \mathit{UPDATE} \,\cup\,\{u\}$;\;}

}

}

}


%$\mathit{DE3} \leftarrow \mathit{DE1}\,\backslash\, \mathit{DE2}$;\;
%\textit{\color{darkgreen} /* Domain Model*/} \;
$\mathit{UPDATE} \leftarrow \mathit{UPDATE}\, \cup\, (\mathit{E1}\,\backslash\, \mathit{E3})$;\;

$\textbf{return} \, (\{\mathit{ADD}\} \, \cup \, \{\mathit{DELETE}\} \, \cup \{\mathit{UPDATE}\})$;\;  








%\textit{\color{darkgreen} /* Reconfiguration of PS Model*/} \;


% Let $VP$ be the set of treated VP;\;
% Let $L$ be the set of pairs of variation points $vp$ and use cases $uc$ such that use cases are essential and they include the variation points, or the variation points are not included by any use case;\;
% 
%$Diff \, \leftarrow$ \textbf{getDifferences}($DM1.VP$, $DM2.VP$);\;
%\While{$L \neq \emptyset$} 
%{
%$dp \in L$; \;
%Let $SUC$ be the set of variant use cases selected in $dp.vp$;\;
%Let $NSUC$ be the set of variant use cases unselected in $dp.vp$;\;
%Let $d$ be the quadruple $(dp.vp, dp.uc, SUC, NSUC)$;\;
%\eIf{($d$ \textbf{satisfies} the cardinality constraints in $dp.vp$)}
%{
%Let $C$ be the empty set for contradicting decisions;\;
%%\textit{\color{darkgreen} /* initialize the set of contradicting decisions*/} 
%$C \leftarrow$ \textbf{checkConflictingVP}($dp.vp$, $DC$, $d$, $PLD$);\;
%$C \leftarrow C\,\cup\,$\textbf{checkRequiringVP}($dp.vp$, $DC$, $d$, $PLD$);\;
%$C \leftarrow C\,\cup\,$\textbf{checkRequiredVP}($dp.vp$, $DC$, $d$, $PLD$);\;
%\ForEach{($u \in SUC$)}
%{
%$C \leftarrow\,C\,\cup\,$\textbf{checkConflictingUC}($u$, $DC$, $d$, $PLD$);\;
%$C \leftarrow\,C\,\cup\,$\textbf{checkRequiringUC}($u$, $DC$, $d$, $PLD$);\;
%}
%
%\ForEach{($u \in NSUC$)}
%{$C \leftarrow C\,\cup\,$\textbf{checkRequiredUC}($u$, $DC$, $d$, $PLD$);\;}
%
%\eIf{($C = \emptyset $)}
%{
%$DC \leftarrow\, DC \cup \{d\}$;\;
%%saveDecision($DM$, $d$); \;
%$L \leftarrow L \backslash \{dp\}$;\;
%%Let $new_{vp}$ be the set of new couples (variation point$\backslash$use case) included by $suc$ $|$ $new_{vp}\,\cap\,L = \emptyset$;\;
%Let $new_{p}$ = $\{ (vp, uc) \, | \, uc \, \textbf{includes} \, vp \, \wedge \, uc \in SUC \, \wedge \, (vp, uc) \notin T\}$;\;
%$L \leftarrow L \cup new_{p}$; \;
%$T \leftarrow T \cup new_{p}$;
%}
%{
%%report inconsistencies of $d$ with regards to the previous decisions in $DM_{PLD}$\;
%%Ask the user to modify their choices\;}
%updateDecisions($C$ $\cup$ \{$d$\});\;} 
%
%}
%%{Ask the user to modify their choices\;}
%{updateDecisions(\{$d$\});\;}
%} 
%
%






\caption{\textit{Diff}}\label{algo:diff}
\end{algo}
\end{tiny}
%\end{minipage}




==> algos/algoreconfig.tex <==


\begin{scriptsize}
\begin{algo} 

\DontPrintSemicolon 
 \SetKwInOut{Input}{Inputs}\SetKwInOut{Output}{Output}
 \SetAlgoLined
  \SetInd{0.6em}{0.6em}
 \setcounter{AlgoLine}{0}
\Input{PS use case diagram, $PSD$,
 Set of PS use case specifications, $PSS$,
 PS domain model, $PSM$, 
 Set of added decisions, $ADD$,
 Set of deleted decisions, $DELETE$,
 Set of updated decisions, $UPDATE$}
 \Output{Set of PS use case models}
 \BlankLine

 %Let $PSD$ be the PS use case diagram; \;
 %Let $PSS$ be the set of PS use case specifications; \;
 %Let $PSDM$ be the PS domain model; \;
 
 %Let \textbf{\textit{updateDecisions}}($D$) be the function where the analyst update one or more decisions in the set of decisions $D$; \;
 
 %Let $DC$ = $\emptyset$; \textit{\color{darkgreen} /* initialize the set of decisions*/} \;
 Let $DC$ be the empty set for completed decisions; \;
 
%Let $DM$ be the decision model \textit{\color{darkgreen} /* $composed~by:$ $DM_{PLD}$, $DM_{PLS}$, and $DM_{PLDM}$ */}\; 
%Let $PSM$ be the set of PS use case models;\;
%\scalebox{0.9}{Let $PSM$ be the set of product specific use case models
% \textit{\color{darkgreen} /* $PSM =$ \{$PSD$\} $\cup$ \{$PSS$\} $\cup$ \{$PSDM$\} $\cup$ \{$DM$\} */}\;}

%Let $EUC$ be the set of essential use cases in $PLD$; \;

%Let $VP$ be the set of variation points either included by an essential use case or not included by any use case; \;
%Let $VP$ = $\{p \, | \, includes(u, p) \wedge (u \in EUC \, \veebar \, u = null)\}$;\;

%Let $UC$ be the set of use cases $u$ such that $u$ \textit{includes} $v \in VP$;\; 
%Let $UC$ = $\{u \, | \, includes(u, p) \wedge p \in VP \wedge u \in EUC\}$;\;

%Let $L$ be the set of pairs of (vp$\backslash$uc) $|$ variation points are not included by any variant use case in $PLD$ \;
%Let $L$ = $\{ (vp, uc) \, | \, vp \in VP \wedge (uc \in UC \, \veebar \, uc = null) \wedge includes(uc, vp) \}$ ;\;
Let $L$ be the set of pairs of variation points $vp$ and use cases $uc$ such that use cases are essential and they include the variation points, or the variation points are not included by any use case; \;
%Let $T$ = $L$; \;
$T \leftarrow L$; \;

%(($L$ \textbf{contains} at least one couple with Mandatory variation point)) \textbf{or} (user \textbf{not} \emph{done} with decisions)
\While{$L \neq \emptyset$} 
{
%Let $dp$ be the decided pair in $L$;\;
$dp \in L$; \;
%Let $suc$ and $nsuc$ be the sets of selected and \emph{not} selected variant use cases in $dp$, respectively;\;
Let $SUC$ be the set of variant use cases selected in $dp$.$vp$; \;
Let $NSUC$ be the set of variant use cases unselected in $dp$.$vp$; \;
%Let $nsuc$ be the set of \emph{not} selected variant use cases in $dp$;\;
Let $d$ be the quadruple $(dp.vp, dp.uc, SUC, NSUC)$;\;
\eIf{($d$ \textbf{satisfies} cardinality constraints in $dp.vp$)}
{
%Let $cd= \emptyset$ ;\;
Let $C$ be the empty set for contradicting decisions; \;
%\textit{\color{darkgreen} /* initialize the set of contradicting decisions*/} 
$C \leftarrow$ \textbf{checkConflictingVP}($dp.vp$, $DC$, $d$, $PLD$);\;
$C \leftarrow C\,\cup\,$\textbf{checkRequiringVP}($dp.vp$,$DC$,$d$,$PLD$);\;
$C \leftarrow C\,\cup\,$\textbf{checkRequiredVP}($dp.vp$,$DC$,$d$,$PLD$);\;
\ForEach{($u \in SUC$)}
{
$C \leftarrow\,C\,\cup\,$\textbf{checkConflictingUC}($u$,$DC$,$d$,$PLD$);\;
$C \leftarrow\,C\,\cup\,$\textbf{checkRequiringUC}($u$,$DC$,$d$,$PLD$);\;
}

\ForEach{($u \in NSUC$)}
{$C \leftarrow C\,\cup\,$\textbf{checkRequiredUC}($u$, $DC$, $d$, $PLD$);\;}

\eIf{($C = \emptyset $)}
{
$DC \leftarrow\, DC \cup \{d\}$;\;
%saveDecision($DM$, $d$); \;
$L \leftarrow L \backslash \{dp\}$;\;
%Let $new_{vp}$ be the set of new couples (variation point$\backslash$use case) included by $suc$ $|$ $new_{vp}\,\cap\,L = \emptyset$;\;
Let $new_{p}$ = $\{ (vp, uc) \, | \, uc \,\, \textit{\textbf{includes}} \,\, vp \, \wedge \, uc \in SUC \, \wedge \, (vp, uc) \notin T\}$;\;
$L \leftarrow L \cup new_{p}$; \;
$T \leftarrow T \cup new_{p}$;
}
{
%report inconsistencies of $d$ with regards to the previous decisions in $DM_{PLD}$\;
%Ask the user to modify their choices\;}
\textbf{updateDecisions}($C$ $\cup$ \{$d$\});\;} 

}
%{Ask the user to modify their choices\;}
{\textbf{updateDecisions}(\{$d$\});\;}
} 

\textbf{... }

%performGeneralCheck($DM$); \textit{\color{darkgreen} /* all unspecified choices will be considered as excluded */} \;

%$PSM =$ \{$PSD$\} $\cup$ \{$PSS$\} $\cup$ \{$PSDM$\} $\cup$ \{$DM$\}\;
%\textbf{return $PSM$}; \;


\caption{\textit{Reconfig}}
\label{alg:reconfig}
\end{algo}
\end{scriptsize}



==> tableExampleInputLogRegr.tex <==

\begin{table}
\scriptsize
\caption{Part of the Example Input for Logistic Regression}
 \vspace*{-1.3em}
\begin{center}
\begin{tabular}{|p{1.0cm}|p{0.95cm}||p{0.6cm}|p{0.60cm}||p{1.70cm}|p{1.45cm}|p{1.20cm}|p{1.42cm}|p{1.42cm}|}

\hline

\textbf{Product ID}&\textbf{Version ID}&\textbf{Test Case ID}& \textbf{Fails}& \textbf{Classification of the Test Case}& \textbf{Size of the Use Case Scenario}&\textbf{Variation in the Scenario}&\textbf{Percentage of Failed Products}&\textbf{Percentage of Failed Versions}\\

\hline
\hline
CH&	V1&	TC1	&	1	&	New	&0.075&0&0.2&0.025\\
CH&	V2&	TC1	&	1	&	New	&0.075&0&0.2&0.025\\
CH&	V3&	TC1	&	0	&	New	&0.075&0&0.2&0.025\\
CH &V4&	TC1	&	0	&	New	&0.075&0&0.2&0.025\\

\hline

CH&	V1&	TC2	&	0	&	New	&0.225&0.03&0.2&0.040\\
CH&	V2&	TC2	&	0	&	New	&0.225&0.03&0.2&0.040\\
CH&	V3&	TC2	&	0	&	New	&0.225&0.03&0.2&0.040\\
CH &V4&	TC2	&	0	&	New	&0.225&0.03&0.2&0.040\\

\hline

SGM& V1& TC1	&	0	&	Retestable	&0.075&0&0.2&0.025\\
SGM& V2& TC1	&	0	&	Retestable	&0.075&0&0.2&0.025\\
SGM& V3& TC1	&	0	&	Retestable	&0.075&0&0.2&0.025\\

\hline

SGM& V1& TC2	&	1	&	Reusable	&0.225&0.03&0.2&0.040\\
SGM& V2& TC2	&	1	&	Reusable	&0.225&0.03&0.2&0.040\\
SGM& V3& TC2	&	0	&	Reusable	&0.225&0.03&0.2&0.040\\

\hline

DM& V1& TC1	&	0	&	Retestable	&0.075&0&0.2&0.025\\
DM& V2& TC1	&	0	&	Retestable	&0.075&0&0.2&0.025\\

\hline

DM& V1& TC2	&	0	&	Retestable	&0.075&0.03&0.2&0.040\\
DM& V2& TC2	&	0	&	Retestable	&0.075&0.03&0.2&0.040\\

\hline

\end{tabular}
\end{center}
\label{table:logisticRegressionInput}
 \vspace*{-1.2em}
\end{table}

